Personalized Chatbot Trustworthiness Ratings

Conversation agents, commonly referred to as chatbots, are increasingly deployed in many domains to allow people to have a natural interaction while trying to solve a specific problem. Given their widespread use, it is important to provide their users with methods and tools to increase users awareness of various properties of the chatbots, including non-functional properties that users may consider important in order to trust a specific chatbot. For example, users may want to use chatbots that are not biased, that do not use abusive language, that do not leak information to other users, and that respond in a style which is appropriate for the user's cognitive level. In this paper, we address the setting where a chatbot cannot be modified, its training data cannot be accessed, and yet a neutral party wants to assess and communicate its trustworthiness to a user, tailored to the user's priorities over the various trust issues. Such a rating can help users choose among alternative chatbots, developers test their systems, business leaders price their offering, and regulators set policies. We envision a personalized rating methodology for chatbots that relies on separate rating modules for each issue, and users' detected priority orderings among the relevant trust issues, to generate an aggregate personalized rating for the trustworthiness of a chatbot. The method is independent of the specific trust issues and is parametric to the aggregation procedure, thereby allowing for seamless generalization. We illustrate its general use, integrate it with a live chatbot, and evaluate it on four dialog datasets and representative user profiles, validated with user surveys.

==> backup.tex <==
\section{Backup - To Be Removed Later}

% In the example of customer support center, a user contacts a service center and enters into a dialog with a customer support agent. The participant roles here are that of a customer and an agent, and the roles inter-leave in every turn. On the other hand, in the example of online support, a person may raise an issue on a public portal and anyone may reply. 



% --------------------
\subsection{Example - Using Dialogs to Find Information Arranged in a Taxonomy}

One popular category of user dialogs in business setting is inquiry of information that is organized in a taxonomy. For instance, a person wants to ask about a product on a company's site (e.g., {\em pliers} - product, job openings) but does not know which particular type. An example of taxonomy is
United Nations Standard Products and Services Code (UNSPSC\footnote{https://www.unspsc.org/}), which {\em "is an open, global, multi-sector standard for efficient, accurate classification of products and services"}. Table~\ref{tab:unspsc} gives a summary of the levels in the taxonomy and its data. There are 4,302 items arranged into class, family, segment and commodity (lowest level). The {\em characteristic} column conveys the nature of abstraction across levels by reporting number of distinct (dissimilar) values, unique (count=1) values and their percentage, followed by highest frequency at a given level. 

So, if the user inquires about a product, the chatbot can refer to the taxonomy to confirm what the user wants. As example,  a query on   {\em pliers} may refer to a surgical tool (Code: 42292303) or a vehicle servicing equipment (Code: 25191716) or a hand tool (Code: 27112106), and many variations therein. Thus, there can be a varieties strategies for a chatbot to help the user. It can go from highest level to lowest, or reverse, or ask randomly from the tree. Furthermore, if there is a restriction on how many turns the chatbot can take on this query, we want to explore if there are  querying strategies that are optimal.
 

% Distinct means the number of dissimilar values contained for the selected attribute. Unique means the number and percentage of instances having a value for this attribute that no other instances have in the data.


% ---------------------

\begin{table}[t!]
\scriptsize
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Level} & \textbf{Name} & \textbf{Characteristic} \\ \hline
\textbf{4 - Highest} & Segment & 36; 3 (0\%); 825  \\ \hline
\textbf{3} & Family & 173; 23 (1\%); 443  \\ \hline
\textbf{2} & Class & 826; 216 (5\%); 49  \\ \hline
\textbf{1 - Lowest} & Commodity & 4302; 4302 (100\%); 1  \\ \hline
\end{tabular}
\caption{Levels in UNSPSC Taxonomy.}
\label{tab:unspsc}
\end{table}
% ---------------------
